Search for anomalous production of events with same-sign dileptons and b jets in 14.3 fb^-1 of pp collisions at sqrt(s) = 8 TeV with the ATLAS detector

A search is presented for exotic processes that result in final states containing jets including at least one b jet, sizable missing transverse momentum, and a pair of leptons with the same electric charge. Using a sample of 14.3 fb^-1 of pp collisions at sqrt(s) =8 TeV recorded by the ATLAS detector at the Large Hadron Collider, no significant excess of events over the background expectation is observed. This observation is interpreted as constraining several signal hypotheses beyond the Standard Model and limits are set at 95% confidence level on relevant parameters of the signal hypotheses.

==> Makefile <==
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = eprint_dpf2013
PDFNAME = eprint_dpf2013.pdf

#default: testlatex
default: testpdflatex

testlatex:
	${LATEX}  ${BASENAME}
	${LATEX}  ${BASENAME}
#	${BIBTEX} ${BASENAME}
#	${LATEX}  ${BASENAME}
#	${LATEX}  ${BASENAME}
#	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME} ${PDFNAME}
#	dvipdfm ${BASENAME}	# did not try dvipdfmx
#	dvips ${BASENAME}

testpdflatex:
	${PDFLATEX} ${BASENAME}
	${PDFLATEX} ${BASENAME}
	${BIBTEX}   ${BASENAME} || echo "Ignoring bibtex errors"
	${PDFLATEX} ${BASENAME}
	${PDFLATEX} ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
#	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
#	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *.lof *.log *.lot *~ ~* spellTmp 


